Future-based Static Analysis of Message Passing Programs

Message passing is widely used in industry to develop programs consisting of several distributed communicating components. Developing functionally correct message passing software is very challenging due to the concurrent nature of message exchanges. Nonetheless, many safety-critical applications rely on the message passing paradigm, including air traffic control systems and emergency services, which makes proving their correctness crucial. We focus on the modular verification of MPI programs by statically verifying concrete Java code. We use separation logic to reason about local correctness and define abstractions of the communication protocol in the process algebra used by mCRL2. We call these abstractions futures as they predict how components will interact during program execution. We establish a provable link between futures and program code and analyse the abstract futures via model checking to prove global correctness. Finally, we verify a leader election protocol to demonstrate our approach.

==> eptcsdata.tex <==
\providecommand{\firstpage}{65}
\providecommand{\publicationstatus}{D. Orchard and N. Yoshida (Eds.): Programming Language Approaches to \\ Concurrency- and Communication-Centric Software (PLACES 2016).\\
EPTCS 211, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.211.7}{10.4204/EPTCS.211.7}}
\pdfoutput=1

